Experimental Security Analysis of the App Model in Business Collaboration Platforms

Business Collaboration Platforms like Microsoft Teams and Slack enable teamwork by supporting text chatting and third-party resource integration. A user can access online file storage, make video calls, and manage a code repository, all from within the platform, thus making them a hub for sensitive communication and resources. The key enabler for these productivity features is a third-party application model. We contribute an experimental security analysis of this model and the third-party apps. Performing this analysis is challenging because commercial platforms and their apps are closed-source systems. Our analysis methodology is to systematically investigate different types of interactions possible between apps and users. We discover that the access control model in these systems violates two fundamental security principles: least privilege and complete mediation. These violations enable a malicious app to exploit the confidentiality and integrity of user messages and third-party resources connected to the platform. We construct proof-of-concept attacks that can: (1) eavesdrop on user messages without having permission to read those messages; (2) launch fake video calls; (3) automatically merge code into repositories without user approval or involvement. Finally, we provide an analysis of countermeasures that systems like Slack and Microsoft Teams can adopt today.

==> src/intro.bak.tex <==
\section{Introduction}

% opening para
% IRC has evolved into slack with many productivity features. Slack, Discord are big players. These platforms have brought benefits like making remote work more productive. The popular slack platform carries a lot of sensitive data and manages access to sensitive resources. security design issues can put all these resources at risk of being accessed by attackers. Slack is the biggest market player, others are MSFT teams and Discord.
Internet Relay Chat (IRC) has evolved into online communication platforms like Slack, Microsoft Teams and Discord. These modern reincarnations of IRC can do a lot more than text-based chatting. They help users share multimedia content, automate tasks~\cite{stuff} and serve as a single centralized hub for managing a diverse set of online resources like cloud storage and video calls~\cite{stuff}. Spurred on by the COVID-19 pandemic and the general shift to remote working, platforms like Slack have solidified their position as critical enabling technology for any type of team-based work environment. For example, in 2020, Slack had more than 12 million daily active users, with 65 of the Fortune-100 companies using Slack as their main workspace communication tool~\cite{slack-stats}. 

% motivation
% talk about recent breaches. 
% To enhance productivity, slack includes a third-party integration model. this enables developers to create new features and extend the slack platform. 
Given the scale of access to sensitive resources, Slack is a target for attackers. For example, the recent breach of Electronic Arts' Slack workspace resulted in attackers stealing 780GB of data including internal source code~\cite{ea-hack}. Meanwhile, to support the growing demand for productivity, Slack is pushing newer features, some of which are not well-designed from a security and privacy perspective, resulting in even more vulnerabilities~\cite{slack-android-password,slack-feature-withdraw}. 

% what we did and why its important
% we peform an experimental security analysis of slack apps/integrations. it is important to do this analysis because the findings from this analysis will help secure online communication platforms in an increasingly online world. Bugs have been discovered in slack, but little to no research has focused on this emerging form of enhancement to slack-like systems.

%% TODO: do we need to motivate more about why we are focusing on app model and what use is the results for defenses?
We contribute to understanding the security and privacy of online communication platforms by performing an experimental security analysis of the Slack third-party integration model. This model allows third-party developers to create and distribute apps\footnote{Formerly, apps were called Slack Bots.} that users can install into their Slack workspaces. Slack apps extend built-in Slack functionality with the goal of enhancing user productivity. Common apps include Google Calendar, Zoom and DropBox; and as of August 2021, the Slack app store hosts more than 2000 apps~\cite{slack-app-directory}. These apps are highly privileged and manage access to all kinds of sensitive resources. Furthermore, they have direct access to messages in Slack channels as well. To the best of our knowledge, our experimental analysis is one of the first to systematically apply adversarial pressure to this third-party integration model. 

% little more detail about what we are doing
% Slack includes a privilege model for its third-party integrations. based on combo of oauth scopes and runtime policy checking. We focus our analysis on this. we explore under the threat model of malicious app. slack allows app installation by administrator of workspace and anyone in workspace if admin allows.
% why is the analysis challenging?
% slack is closed source; apps are blackbox - no access to source code; so no binary analysis possible; privilege model description is not complete. 

% The security model specifies that a Slack workspace administrator can always install apps from any source, including unofficial sources. Furthermore, the administrator can configure the system to allow any existing user to install an app.

Slack includes a security model for third-party integrations. It is based on a combination of OAuth scopes and runtime policy checks. We focus our analysis on the security model under the attacker assumption of a malicious app that a user has unwittingly installed, a common assumption in app-based security analyses.   
%Once an app is installed, it is available for everyone in the workspace. 
Performing this analysis is challenging for several reasons. First, Slack is a closed-source system, precluding analysis techniques that have been used in open-source systems like Android.  Second, the third-party apps are essentially third-party web services executing on external (to Slack) cloud infrastructure that invoke Slack-defined web APIs to interact with Slack-managed resources. This precludes analysis techniques that require source code or binary access to the apps. Furthermore, the API endpoints are hidden and only known to the Slack server, preventing us from directly exercising app behavior. Rather, we are confined to the interfaces that Slack provides, such as sending a message to the Slack app. The third challenge is that the privilege model is not fully specified in the Slack documentation --- without a complete specification, it is not possible experimentally evaluate security comprehensively.


% how do we overcome challenges? what's our methodology?
% build prototype apps to manually exercise slack app features or all aspects of its app security model?
We overcome these challenges using a combination of manual analysis and automated measurements. Specifically, we derive a more complete privilege model for Slack apps. 
Using our manually created test apps with varying degrees of permissions, we queried various resources in a workspace to exercise the privilege checking logics of different Slack APIs. We found that, to determine whether an app has the correct privilege to access a resource, Slack generally goes through two levels of checking: first, it verifies whether the app has the OAuth scopes required to access this type of resources; second, it uses a number of customized runtime rules to control, out of all instances in this resource type, which ones can be accessed by the app, based on the attributes of each instance.

%Using that more complete specification, we manually create test Slack apps to exercise the security model. 
%\ef{needs more meat here.}

% overview the findings. stress that we uncover fundamental design weaknesses.
% attack type 0: user delegation confuses runtime policy checking: app can act as user or app itself. 
% attack type 1: security model incompleteness. combining two permissions yields more abilities than the sum of those permissions.
% attack type 2: namespace collisions allow command hijacking.

\noindent\textbf{Our Contributions.} We discovered security-critical design flaws in three areas of the Slack security model: malicious app-to-app interactions, command namespace collisions and insufficient runtime policy checks. Together, these issues undermine the confidentiality and integrity of resources that a user entrusts with Slack. 

\begin{itemize}
    \item \textit{Malicious App-to-App Interactions:}
    
    We found that Slack apps can interact with each other in malicious ways. Coupled with the feature of an app to behave like a human user, this can lead to confidentiality and integrity violations. For example, a malicious app may masquerade as a human user and send a Slack message to a victim app (e.g., Dropbox or Email) and get it to perform actions that the user did not expect. This design flaw stems from the fundamental lack of semantic context for a security system to make a judgement about whether certain interactions are legitimate and align with user expectations. In some cases, an app-to-app interaction offers useful functionality such as automating a task. For example, when DropBox shares contents to Slack channels as the user, another app called Dokkio~\cite{dokkio} can subsequently organize such contents into a coherent page and tags them as shared by the user. In other cases, this interaction is unwanted. We show that this design issue is exploitable by creating four proof-of-concept attacks where a malicious Slack app can: (1) send emails on a victim user's behalf; (2) retweet on a victim user's behalf; (3) reply to comments on a Google document; and (4) add files to a cloud file management portal. In all cases, the attacker does not have the permission to perform such activities on the victim user's behalf.
    
    \item \textit{Command Namespace Collisions:}
    
    Slack apps provide commands (e.g., \texttt{/zoom} to start a video call). We find that all these command share a single namespace, allowing collisions. A malicious app can create a command to collide with an existing one from a different app and then \textit{override} it so that the malicious command gets executed. Naming collisions are a design issue that plague many systems, including DNS and more recently, voice assistants like Alexa~\cite{skill-squat}. We show this issue is exploitable by creating a malicious Zoom command that replaces a victim's video call with one that an attacker has access to. This can lead to confidentiality violations. 
    
    \item \textit{Insufficient Runtime Policy Checks:}
    
    Slack uses a combination of OAuth scopes requested at development time and runtime policy checks to implement the app security model. For example, an app can request an OAuth token to read private messages at development time. Later at runtime, a user has to add that app to a private channel for it to access private messages. Whenever the app sends an API request to the Slack server to read a message, Slack has to verify the OAuth token scope and separately check that the app was added to the channel it is trying to read from. This design choice of having context-specific security checks is prone to being incomplete because some checks can be missed. We show that this design issue is exploitable by creating a malicious app that leaks messages in private Slack channels \textit{without} the permission to read from those channels.

\end{itemize}

% discuss measurements.
% \ef{TODO: discuss something about measurements we've done and how it supports the above findings.}
We measure the prevalence of the potential for the above attacks to occur by analyzing the permissions of all 2,640 apps in the Slack app store. We find that 53\% of apps have the potential to interact adversarially with other apps if they choose to, whereas, 61\% of apps are potentially vulnerable to such interactions. Furthermore, we find that 51\% of apps use the command feature and thus sharing the same command namespace, opening up the possibility for attackers to adversarially override benign commands.

%of the above design issues across all 2,460 public apps in the Slack App Directory.  For example, 53\% of apps can interact with other apps adversarially if they choose to, whereas 61\% of apps are potentially vulnerable to such interactions if not properly handled their resources. Furthermore, we discover that over 51\% of apps share the same command namespace, allowing them to overwrite one other's commands adversarially.

% ending para: broader impacts
Finally, we discuss countermeasures that Slack can implement to avoid the above design issues.  For example, enforcing user confirmation before every app-to-app interaction and command name collision can fix most issues, but this is undoubtedly a user-hostile solution. As a result, solutions with acceptable security and usability trade-offs would necessitate rethinking access control design in multi-user communication and productivity platforms like Slack. %\ef{make more concrete.}

\paragraph{Ethics and Disclosure.} We conducted all experiments inside a private workspace with the authors as the only members. We did not exercise cross-workspace features, thus, our investigations did not influence other workspaces. We did not distribute or submit our experimental malicious apps to Slack's app directory, so our attack did not affect Slack users other than the authors. At the time of submission, we have initiated a vulnerability disclosure with the Slack security team.




==> src/intro.tex <==
\section{Introduction}\label{sec:intro}

Business collaboration platforms (BCPs), such as Slack, Microsoft Teams, and Discord, enhance collaboration and productivity through \emph{third-party apps}. Developers create and distribute third-party apps that add specialized features to BCP's built-in functionalities beyond text-based chatting. There are apps for interacting with Google Calendar, making video calls with Zoom, and even accessing Dropbox files directly from the platform. To support these collaborative and productive features, BCPs not only host users' private communications but also facilitate access to other sensitive resources. However, the execution of security principles behind these features is unknown, resulting in additional security vulnerabilities~\cite{slack-android-password,slack-feature-withdraw}.

In this paper, we perform the first experimental security analysis of the third-party app model in BCPs. Performing this analysis is challenging in two folds. First, third-party apps are proprietary web services, preventing traditional security analyses based on source code or binaries. Second, the app's API endpoints are secret and only known to the BCP server, precluding direct security testing of the apps' web endpoints. To overcome these challenges, we focus on \emph{interactions} that an app can receive or initiate through BCPs, such as sending chat messages and reacting to messages. Guided by our systematized app permission model and security principles that apply the most in the context of BCPs, we build a set of test apps to analyze all interactions between apps and users, and then exercise security principles to find violations. 

% Business collaboration platforms (BCPs) like Slack, Microsoft Teams, and Discord
% provide text-based chatting features --- like Internet Relay Chat
% (IRC)~\cite{oikarinen1993internet} --- and much
% more.
% They help users share multimedia content, automate tasks~\cite{slack-workflow}, and serve
% as a single centralized hub for managing a diverse set of online resources like
% cloud storage and video calls~\cite{slack-ad-1, slack-ad-2}. Spurred on by the COVID-19 pandemic
% and the general shift to remote working, BCPs have solidified
% their position as critical technology for team-based work
% environments. For example, in 2020, Slack had more than 12~million daily active
% users, with 65 of the Fortune-100 companies using Slack as their main
% communication tool~\cite{slack-stats}.


% Many of these platforms allows integrating with third-party apps
% To enhance user experience and productivity, these platforms allow third-party developers to
% create and distribute apps
% that
% extend their built-in functionalities with specialized features. 
% There are apps for interacting with Google Calendar, creating
% video calls with Zoom, and even accessing files on Dropbox directly within
% the platform. As of August 2021, the Slack app store, for instance, hosts more than 2,640
% official apps~\cite{slack-app-directory}, with many more unofficial apps listed on sites like GitHub.  Thus,
% these platforms not only host users' sensitive communications but also facilitates access to other sensitive resources such as calendars, cloud storage, and even financial information through third-party apps.


% Given the sensitive resources that BCPs have access to, they are
% regularly targeted by attackers.  For example, the recent breach of Electronic
% Arts' Slack workspace resulted in attackers stealing 780GB of data including
% internal source code~\cite{ea-hack}.  Moreover, they provide complex and rich
% interactions between users and apps, which could lead to additional security
% vulnerabilities~\cite{slack-android-password,slack-feature-withdraw}.

% , to support the growing demand for
% productivity, Slack is also trying newer features with less comprehensive
% security and privacy analysis, % some of which could be not well-designed from a
% % security and privacy perspective,
% leading to even more

% In this paper, we perform the first experimental security analysis of the third-party app model in business communication platforms. We focus
% on the app model because it is a primary feature that allows third-parties to extend functionality and enhance user productivity. Performing this analysis is challenging because third-party apps are proprietary web services. Thus, traditional security analyses based on source code or binaries cannot be used for these apps. Furthermore, the app's API endpoints are hidden and only known to the platform server, precluding direct security testing of the apps' web endpoints. Therefore, we focus on \emph{interactions} that an app can receive or
% initiate through communication platforms. Our methodology is to list all interactions between apps and users (e.g., sending chat messages, reacting to messages) and build a set of test apps to exercise security principles with the goal of finding violations. 

%a widely-used app-enabled online
%communication platform such as Slack by conducting a security
%analysis of Slack's third-party app model.  % Due to closed source nature of Slack
% it's apps, traditional security analysis that require source code or binary
% will not work in this context.

% Therefore, we focus on \emph{interactions} that an app can receive or
% initiate through communication platforms. Once installed in a workspace, an app can interact with the platform
% server, with users in the workspace, and even with other third-party apps. Our methodology is to list all interactions between apps and users (e.g., sending chat messages, reacting to messages) and build a set of test apps to exercise the platform's security policy with the goal of finding violations.


We discover that both Slack and Microsoft Teams violate two fundamental security principles: \emph{least privilege} and \emph{improper tracking of resource ownership}. According to our analysis of the app permission model in BCPs, these platforms implement runtime policy checks on the static OAuth scopes to support flexible permission control. However, the adopted runtime checks are typically incomplete due to a lack of understanding of the user's intention. The acquisition of such knowledge is subject to an unfavorable trade-off between security and usability. As a result, we identify two security-critical design flaws in their third-party app model: the \emph{app-app} interaction and the \emph{app-user} interaction.

% We discovered security-critical design flaws in all three types of interactions in Slack's
% third-party app model: app-to-app, user-to-app, and
% app-to-user interaction.

%\begin{newitemize}
\vspace{2pt}
\noindent\textit{(1) App-app:} Apps interact with other entities in a workspace through multiple ways such as sending a chat message or reacting to a chat message with emojis. 
Such interactions can be very useful for automating tasks. For these
interactions, apps require a user-delegation token that allows them to perform
actions on behalf of a user. However,
such a %provides the app with such a token,
user-delegation token also enables the app to interact with \emph{any other} app
in the workspace without restriction. Thus, a malicious app with a user-delegation token can interact with another (victim) app by sending messages
 without the user's consent.  %\fixme{This design flaw stems from the
%  fundamental lack of semantic context for an access control system}
Victim apps often lack the semantic context necessary to judge whether certain interactions are legitimate and align with user
expectations. We exploit this design issue by creating four proof-of-concept
attacks. For example, we show that one can send emails on behalf of an
unsuspecting user by exploiting the MailClark app in Slack.
  

\vspace{2pt}    
\noindent\textit{(2) App-user:} Apps and users interact with each other from both sides. On one side, users directly interact with apps by either \emph{mentioning} the app user with `\codefont{@}' prefix or typing a \emph{slash command} with `\codefont{/}' prefix. For example, one can start a Zoom video call by entering \codefont{/zoom} on the Slack UI. The Slack server interprets the
  commands and notifies a specific app (e.g., Zoom, in this case) that registered
  the command. However, we found that all these commands share a single
  namespace, and that collisions can override the apps that get notified.  
  Similar naming collisions are a design issue that plagues many systems,
  including %, including DNS and more recently,
  voice assistants like Alexa~\cite{kumar2018skill,zhang2019dangerous}. We exploit this issue by creating a malicious app overriding the \codefont{/zoom}
  command that replaces a victim's video call link with one that the attacker
  controls.

On the other side, apps interact with users on
  Slack by participating in any approved channels or conversations, where a human participant explicitly `adds' the app as a member. Slack implements runtime policy checks to enforce security policies in these situations. For example, an app can request an OAuth token to read private messages
   at development time. Later at runtime, a user has to add that app to a private
   channel for it to access private messages. Whenever the app sends an API
   request to the Slack server to read a message, Slack has to verify the OAuth
   token scope and separately check that the app was added to the channel it is
   trying to read from. This design choice of having context-specific security
   checks are prone to being incomplete. We show
   that this design issue is exploitable by creating a malicious app that leaks
   messages in private Slack channels \textit{without} the permission to read
   from those channels.


% \vspace{2pt}    
% \noindent\textit{(2) App-user:} Users can directly interact with apps
%   by either mentioning the corresponding ``app user'' (a.k.a, ``bot user'') with
%   `\codefont{@}' prefix, or by typing a \emph{slash command} (which always
%   starts with a slash `\codefont{/}').  For example, one can start a Zoom video
%   call by entering \codefont{/zoom} on the Slack UI. The Slack server interprets the slash
%   commands and sends a notification to a specific app (e.g., Zoom, in this case) that registered
%   the command. However, we found that all these slash commands share a single
%   namespace, and that collisions can override the apps that get notified.  
%   Thus, a malicious app installed in the workspace can
%   hijack user-to-app interaction by creating a command (e.g.,
%   \codefont{/zoom}) that is used by another app. The user has no simple way to
%   find out that the app they are interacting with is not the legitimate app, and
%   therefore can be easily phished for sensitive information, such as passwords.

%   Similar naming collisions are a design issue that plagues many systems,
%   including %, including DNS and more recently,
%   voice assistants like Alexa~\cite{kumar2018skill,zhang2019dangerous}. We show that this issue is
%   exploitable by creating a malicious app overriding the \codefont{/zoom}
%   command that replaces a victim's video call link with one that the attacker
%   controls. %(More details in~\Cref{sec:user-to-app}.)
    
% \vspace{2pt}
% \noindent\textit{(3) App-to-user:} 
% An app can interact with users on
%   Slack by participating in any approved (public or private) channels or
%   conversations. An approved channel or conversation is one where a human participant explicitly `adds' the app as a member. To enforce security policies in these situations, Slack implements runtime policy checks. For example, an app can request an OAuth token to read private messages
%   at development time. Later at runtime, a user has to add that app to a private
%   channel for it to access private messages. Whenever the app sends an API
%   request to the Slack server to read a message, Slack has to verify the OAuth
%   token scope and separately check that the app was added to the channel it is
%   trying to read from. This design choice of having context-specific security
%   checks are prone to being incomplete. We show
%   that this design issue is exploitable by creating a malicious app that leaks
%   messages in private Slack channels \textit{without} the permission to read
%   from those channels.
  
  
  

% \vspace{1mm}
% We believe the implications of our work relate broadly to the security design of chat-based online communication and productivity tools. The three platforms we study use a similar app model where third-party apps are web services that use OAuth tokens. They also have a similar concept of channels (including private ones) and app commands. We leave analyzing other specific systems to future work, however, the findings here are a potential roadmap for those investigations. 

\paragraph{Contributions.}  %The main contributions of this work are:
\begin{newitemize}
\item We perform the first experimental security analysis of complex interactions between apps and users in popular online communication platforms. Our methodology is to systematize their privilege model and then verify security principles with experimental apps. We discover the violation of two primary security principles, including \emph{least privilege} and \emph{improper tracking of resource ownership}, which lead to real-world confidentiality and integrity attacks.

  
%   \begin{newenumerate}
%   \item Slack allows apps to interact with each other to achieve better productivity. However, coupled with the feature of apps acting on user's behalf, malicious apps can exploit victim apps and make them perform actions the user did not intend.
%     % This is a direct consequence of the OAuth permission model, where, by definition, a token bearer acts like a user from the perspective of the resource provider.
%     It is difficult for apps % access control system
%     to distinguish between malicious and legitimate interactions because it lacks context about what these interactions achieve and whether they align with user expectations.
    
%     %Slack permits apps to act on a user's behalf. This is a direct consequence of the OAuth permission model, where, by definition, a token bearer acts like a user from the perspective of the resource provider. Coupled with the ability for apps to interact with each other directly, malicious apps can masquerade as a human user and issue unwanted instructions to other apps. It is difficult for an access control system to distinguish malicious and legitimate interactions because it lacks context about what these interactions achieve and whether they align with user expectations.
    
%   \item Slack slash commands share a single namespace but allow multiple apps
%     to register the same command.  An attacker can maliciously override the commands of
%     other apps at any time after installation and hijack the messages intended
%     for those
%     apps. % Broadly, this issue occurs in systems where naming a resource has security consequences.
    
%     \item Slack's security policy is incomplete. We show two instances where a set of permissions can be combined to escalate privileges and steal messages in private channels. This issue stems from the challenge of enforcing security policies in environments with dynamic resources.
    
%     %managing permissions in a multi-user environment with dynamic resources.
%   \end{newenumerate}
  
%\item By systematically analyzing the different interactions between apps and
%  other entities in the Slack ecosystem, such as Slack server, users, and other
%  apps, we identify three security issues.  We demonstrate the issues by
%  creating prof-of-concept malicious apps, that we submit to Slack as a part of
%  vulnerability disclosure.
  
  
\item We estimate the prevalence of % the potential for
  apps that have the potential to launch such attacks to occur by analyzing the permissions of all 2,640 apps in the Slack app store. We find that 23\% of apps have the potential to interact adversarially with other apps if they choose to, whereas, 61\% of apps are potentially vulnerable to such interactions. Furthermore, we find that 51\% of apps use the command feature and thus share the same command namespace, opening up the possibility of adversarial overrides. We find that 150 commands are used by multiple published apps with conflicts.
  
  %\ef{should we reword to include anything from latest experiments?}


%We performed a measurement study of the Slack app store to estimate the number of apps that are potential attackers or victims.  We find that approximately 53\% of apps are potentially vulnerable to the attacks, while 67\% can act as potential
%  attackers. We include an exploration of defenses for these exploitable design issues.
  
\end{newitemize}

% As a first of its kind study to analyze the appificed online communication
% platforms, we don't claim that our analysis is exhaustive. However, our work
% should initiate research on how to analyze such systems and 

Finally, we discuss countermeasures that these platforms can implement to avoid the above design issues.  For example, enforcing user confirmation before every app-app interaction and command name collision can fix most issues, but this is undoubtedly a user-hostile solution. As a result, solutions with acceptable security and usability trade-offs would necessitate rethinking the app and access control model in multi-user communication platforms.

%access control design in multi-user communication and productivity platforms like Slack.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

%  LocalWords:  workspaces




%We find that certain interactions entail fundamental design issues that an attacker can exploit. Specifically, we find security-critical design issues in all interactions between users and apps.

%systematically analyze the security issues that could arise in these interactions and show that certain interactions entail fundamental
%design issues that an attacker can
%exploit. % Apps can only interact through the Slack server, thus the Slack can
% always employ the permission check. 


% We contribute to understanding the security and privacy of online communication platforms by performing an experimental security analysis of the Slack third-party integration model. 

% Taking Slack as a case in point, we aim to understand the challenges in
% instantiating a secure multi-user authorization model with third-party app
% integration. 

% Slack includes a security model for third-party integrations. It is based on a combination of OAuth scopes and runtime policy checks. We focus our analysis on the security model under the attacker assumption of a malicious app that a user has unwittingly installed, a common assumption in app-based security analyses.   
% %Once an app is installed, it is available for everyone in the workspace. 
% Performing this analysis is challenging for several reasons. First, Slack is a closed-source system, precluding analysis techniques that have been used in open-source systems like Android.  Second, the third-party apps are essentially third-party web services executing on external (to Slack) cloud infrastructure that invoke Slack-defined web APIs to interact with Slack-managed resources. This precludes analysis techniques that require source code or binary access to the apps. Furthermore, the API endpoints are hidden and only known to the Slack server, preventing us from directly exercising app behavior. Rather, we are confined to the interfaces that Slack provides, such as sending a message to the Slack app. The third challenge is that the privilege model is not fully specified in the Slack documentation --- without a complete specification, it is not possible experimentally evaluate security comprehensively.


% % how do we overcome challenges? what's our methodology?
% % build prototype apps to manually exercise slack app features or all aspects of its app security model?
% We overcome these challenges using a combination of manual analysis and automated measurements. Specifically, we derive a more complete privilege model for Slack apps. 
% Using our manually created test apps with varying degrees of permissions, we queried various resources in a workspace to exercise the privilege checking logics of different Slack APIs. We found that, to determine whether an app has the correct privilege to access a resource, Slack generally goes through two levels of checking: first, it verifies whether the app has the OAuth scopes required to access this type of resources; second, it uses a number of customized runtime rules to control, out of all instances in this resource type, which ones can be accessed by the app, based on the attributes of each instance.

% %Using that more complete specification, we manually create test Slack apps to exercise the security model. 
% %\ef{needs more meat here.}

% Overview The Findings. stress that we uncover fundamental design weaknesses.
% attack type 0: user delegation confuses runtime policy checking: app can act as user or app itself. 
% attack type 1: security model incompleteness. combining two permissions yields more abilities than the sum of those permissions.
% attack type 2: namespace collisions allow command hijacking.

% \paragraph{Our contributions.}




%Slack provides a \emph{self direct-message channel} (which we refer
  %to as the ``self channel'') where the user is the only participant. This self
  %channel is by default approved for any app with the required read
  %(\codefont{im:history}) and write (\codefont{chat:write}). Slack provides
  %another feature called \emph{link unfurling}, that fetches 4000
  %characters of text form a link (including a link to a Slack message) posted on
  %a channel, if all the users in the channel are allowed to view that link. Thus
  %if a link to a Slack message is posted on a self channel the it will be
  %unfurled if the message belongs to a channel which the user is part of.
  %Combining this link unfurling feature on self channel with the ability to read
  %the self channel, a malicious app can read private messages if they can guess
  %the link to Slack messages. We show that it is possible guess links to Slack
  %messages with high probability, allowing an malicious app to read messages in
  %private channels that the app is not even part of.
  %\rahul{This description need another reading.}

  % Interestingly, we found Slack allows users to direct
  % message themselves in a special ``self'' channel, which ideally the user
  % should only be allowed to read and write. However, apps with the permissions
  % mentioned above can also message and read that channel. Apps must be added by
  % the user to a private channel to allow it to read the messages in the private
  % channel. However, a user can post the link to the private channel on their we
  % show that with these permissions an app can read messages from any private
  % channel


% or Slack uses a combination of OAuth scopes requested at
%   development time and runtime policy checks to implement the app security
%   model. For example, an app can request an OAuth token to read private messages
%   at development time. Later at runtime, a user has to add that app to a private
%   channel for it to access private messages. Whenever the app sends an API
%   request to the Slack server to read a message, Slack has to verify the OAuth
%   token scope and separately check that the app was added to the channel it is
%   trying to read from. This design choice of having context-specific security
%   checks is prone to being incomplete because some checks can be missed. We show
%   that this design issue is exploitable by creating a malicious app that leaks
%   messages in private Slack channels \textit{without} the permission to read
%   from those channels.
%\end{newitemize}

% discuss measurements.
% \ef{TODO: discuss something about measurements we've done and how it supports the above findings.}


%of the above design issues across all 2,460 public apps in the Slack App Directory.  For example, 53\% of apps can interact with other apps adversarially if they choose to, whereas 61\% of apps are potentially vulnerable to such interactions if not properly handled their resources. Furthermore, we discover that over 51\% of apps share the same command namespace, allowing them to overwrite one other's commands adversarially.

% ending para: broader impacts
%Finally, we discuss countermeasures that Slack can implement to avoid the above design issues.  For example, enforcing user confirmation before every app-to-app interaction and command name collision can fix most issues, but this is undoubtedly a user-hostile solution. As a result, solutions with acceptable security and usability trade-offs would necessitate rethinking access control design in multi-user communication and productivity platforms like Slack. %\ef{make more concrete.}



  %Although the messages reveal that they were sent by an
  %app on behalf of the user (and not by the users themselves), in the current Slack
  %APIs the identity of the app is not communicated. Thus the victim app has no
  %way to separate the apps with malicious intent from the apps with legitimate
  %intents.
  % This feature We found that Slack apps can
  % interact with each other in malicious ways. Coupled with the feature of an app
  % to behave like a human user, this can lead to confidentiality and integrity
  % violations. For example, a malicious app may masquerade as a human user and
  % send a Slack message to a victim app (e.g., Dropbox or Email) and get it to
  % perform actions that the user did not expect. This design flaw stems from the
  % fundamental lack of semantic context for a security system to make a judgement
  % about whether certain interactions are legitimate and align with user
  % expectations. In some cases, an app-to-app interaction offers useful
  % functionality such as automating a task. For example, when DropBox shares
  % contents to Slack channels as the user, another app called
  % Dokkio~\cite{dokkio} can subsequently organize such contents into a coherent
  % page and tags them as shared by the user. In other cases, this interaction is
  % unwanted. 
   % (1) send emails on a
  % victim user's behalf; (2) retweet on a victim user's behalf; (3) reply to
  % comments on a Google document; and (4) add files to a cloud file management
  % portal. In all cases, the attacker does not have the permission to perform
  % such activities on the victim user's behalf.

==> src/old1_introduction.tex <==
\section{Introduction}

\yue{(note) emphasize design issues, not implementation bugs.}



Slack is a multi-platform online-based business communication platforms that offer Internet Relay Chat style features. A user of Slack can invite a group of people, such as a company or a research group, to join a \emph{workspace}. Inside the workspace, users can create chat rooms, or \emph{channels}, to host conversations in different topics or among different users. 
Incentivized by the shift to remote working during COVID-19 quarantine period, the demand for online workspace communications has grown significantly and so has the usage of Slack. In 2020, Slack is reported to have more than 12 million daily active users and 65 of the Fortune 100 companies are using Slack as their workspace communication tool~\cite{slack-stats}. 

However, Slack, while enjoying their strong growth, is haunted by a series of security and privacy concerns. As more people and companies are using Slack, the amount of sensitive information exchanged through Slack channels has also increased dramatically, making it an attractive target for attackers. One recent breach of Electronic Arts' Slack channel allowed hackers to steal 780GB of data, including many of the company's internal source code~\cite{ea-hack}. Meanwhile, Slack is consistently pushing new features to its clients, trying to satisfy various users' needs and staying ahead of its competitors. Unfortunately, some of these features are not well-designed with carefully considerations in security and privacy, opening up new vulnerabilties~\cite{slack-android-password, slack-feature-withdraw}. 

In this paper, we perform an in-depth study at one of Slack's crucial features --- \emph{Slack apps}. Slack apps\footnotemark, or formerly  known as Slack bots, are third-party integrations that users can install to a workspace. They extend upon existing Slack built-in functionalities and provide connections to other online services, such as Google Calendar and Zoom. As of August 2021, Slack offers more than 2000 apps in its official app directory~\cite{slack-app-directory} and also supports installation of arbitrary unofficial apps. Many of these apps are highly privileged, capable of accessing all kinds of sensitive information including message logs in private, invite-only channels. Therefore, they pose a great security and privacy risk.
In addition, we find some of Slack's design choices, such as hiding the installation process, only escalate such risks.
 

\footnotetext{To avoid ambiguity, we refer to the official Slack client application (which can be either a web browser or a desktop/mobile application) that directly interacts with the users as the Slack \emph{client}.}


We have provided a privilege model for Slack apps, which analyzes how Slack determine whether an app has the correct privilege to access a resource in a workspace. It constitutes two parts: a standardized static scoping checking and customized runtime policy checks. Although Slack does have a rather fine-grained OAuth scopes in place to limit the power of apps (which are significantly better than its competitors like Discord), we still find flaws in the  design of its runtime policy checks part. Specifically, we explore the attack space under the threat model where when a malicious app  is installed in a targeted workspace. 
We are able to create two types of attacks: 

\begin{enumerate}
	\item The first one aims at other benign apps. By taking advantages of resources that Slack's privilege model fail to cover correctly, this type of attacks can impersonate as human users to activate other apps' functionality or steal other apps' commands. 
	\item The second one aims at user's private messages. This type of attacks completely circumvents Slack's privilege model to achieve privilege escalation. We show that it can read messages, including the ones in user's private channels, even without requiring the malicious app to acquire the corresponding permissions.
\end{enumerate}

Finally, for each attack, we surveyed the official Slack App Directory to understand its prevalence, including the number of apps capable of performing the attack and (if applicable) the number of apps susceptible to the attack. We also purpose a number of possible countermeasures for each attack and conclude that to completely prevent these attacks Slack needs to revamp how it models different resources and impose more precise runtime policy checks conditions. 


%the demand for Slack have grown significantly. In 2020, Slack is reported to have more than 12 million daily active users and 65 of the Fortune 100 companies are using Slack as their workspace communication tool~\cite{slack-stats}. Therefore, lots of sensitive information are exchanged through Slack messages.
%One recent breach of Electronic Arts' Slack channel allowed hackers to steal 780GB of data, including many of the company's internal source code~\cite{ea-hack}.
%
%On the other hand, Slack is integrated with a plethora of third-party services, by offering more than 2000 apps in its official app directory. Many of these apps are highly privileged, capable of accessing  \yc{todo: find some concrete examples}.
%


\paragraph{Ethics.}
We did all of our testings and attacks inside our own workspace, where the authors are the sole members.  Since we did not utilize Slack's cross-workspace features, our experiments has no influence on other workspaces.  Therefore, no real Slack users or apps are affected during this study.
As the time of submission, we are currently in the process of communicating with Slack's security team to report our findings.


\yue{explain the challenge: black-box, what we have is already valuable}

\yue{explain how we evaluate the security issues: given features and known security problems, we are evaluating these problems.}

\yue{we are evaluating \textbf{commonly used} features: how many apps have used these features, which features are default, use some results from the measurements.}

\yue{stress that these features increase productivity}

\yue{we don't know the app's impl, we measure how many apps are potentially vulnerably, by counting how many apps have the ability to react to our exploited actions.}

\yue{explain how many apps we tested, and how many works; the number is only an upper-bound, one limitation is that, only a few apps respond to writable scopes.}

\yue{motivate that, the indication of identity is not a good countermeasure, because it is difficult to determine if an event from impersonated user is good or bad. add a screenshot to show legitimate use case.}

